SeqMix: Augmenting Active Sequence Labeling via Sequence Mixup

Active learning is an important technique for low-resource sequence labeling tasks. However, current active sequence labeling methods use the queried samples alone in each iteration, which is an inefficient way of leveraging human annotations. We propose a simple but effective data augmentation method to improve the label efficiency of active sequence labeling. Our method, SeqMix, simply augments the queried samples by generating extra labeled sequences in each iteration. The key difficulty is to generate plausible sequences along with token-level labels. In SeqMix, we address this challenge by performing mixup for both sequences and token-level labels of the queried samples. Furthermore, we design a discriminator during sequence mixup, which judges whether the generated sequences are plausible or not. Our experiments on Named Entity Recognition and Event Detection tasks show that SeqMix can improve the standard active sequence labeling method by $2.27\%$--$3.75\%$ in terms of $F_1$ scores. The code and data for SeqMix can be found at https://github.com/rz-zhang/SeqMix

==> algorithm.tex <==
%%%%%%%%%%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%5%
\begin{algorithm}[htbp]
\label{algo:active_learn}
\SetAlgoNoLine
\textbf{Input}: 
Labeled seed set $\mathcal{L}$;
Unlabeled set $\mathcal{U}$;
Query policy $\psi(\cdot)$;
The sequence labeling model $\theta$.\\
\textbf{Initialization}:\\
 \quad\quad $\theta$ = train ($\theta, \mathcal{L}$)\\
 \While{not stopping criterion}
 {
 // \textit{\textbf{query the unlabeled set and make corresponding annotation $\mathbf{y}$ to expand the training set}}\\
 $\mathcal{L} = \mathcal{L} \cup \left\langle \psi(\mathcal{U}), \mathbf{y} \right\rangle$\\
 $\theta$ = train ($\theta, \mathcal{L}$)\\
 $\mathcal{U} = \mathcal{U} - \psi(\mathcal{U})$\\
 }
 \textbf{Output}:
 Active learned sequence model: $\theta$
 \caption{Pool-based active learning}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%5%

%%%%%%%%%%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%5%
\begin{algorithm}[htbp]
%\label{algo:augmation}
\SetAlgoNoLine
\textbf{Input}: 
Labeled seed set $\mathcal{L}$;
Unlabeled set $\mathcal{U}$;
Query policy $\psi(\cdot)$;
The sequence labeling model $\theta$;
Beta distribution parameter $\alpha$;
Paring method $\zeta(\cdot)$; Discriminator function $d(\cdot)$; Number of expected generation $N$.\\
\textbf{Initialization}:\\
 \quad\quad $\theta$ = train ($\theta, \mathcal{L}$)\\
 \While{not stopping criterion}
 {
 $\mathcal{L} = \mathcal{L} \cup \left\langle \psi(\mathcal{U}), \mathbf{y} \right\rangle$\\
  $\mathcal{U} = \mathcal{U} - \psi(\mathcal{U})$\\
 $\mathcal{L}^* = \textit{SeqMix}(\mathcal{L}, \alpha, \zeta(\cdot), d(\cdot))$\\
 $\mathcal{L} = \mathcal{L} \cup \mathcal{L}^*$\\
 $\theta$ = train ($\theta, \mathcal{L}$)\\
 }
 \textbf{Output}:
The sequence model trained with active data augmentation: $\theta$
 \caption{\\Active augmentation with SeqMix}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%5%

%%%%%%%%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{algorithm}[htbp]
%\label{algo:seqmix}
\SetAlgoNoLine
\textbf{Input}: 
Labeled set $ \mathcal{L} = \left\langle \mathbf{X}, \mathbf{y} \right\rangle$;
Beta distribution parameter $\alpha$;
Paring method $\zeta(\cdot)$; Discriminator function $d(\cdot)$; Number of expected generation $N$.\\
\For {$\left\langle \mathbf{x_i, y_i} \right\rangle, \left\langle \mathbf{x_j, y_j} \right\rangle, (i\neq j) $ in $\mathcal{L}$}
    {
    \If {$\zeta(\left\langle \mathbf{x_i, y_i} \right\rangle, \left\langle \mathbf{x_j, y_j} \right\rangle)$}
        {   
            $\lambda \sim Beta(\alpha, \alpha)$\\
            // \textit{\textbf{mixup the target sub-sequence}}\\
            $\tilde{\mathbf{x_{\textit{sub}}}}=\lambda \mathbf{x_{i\textit{sub}}}+(1-\lambda) \mathbf{x_{j\textit{sub}}}$\\
            $\tilde{\mathbf{y_{\textit{sub}}}}=\lambda \mathbf{y_{i\textit{sub}}}+(1-\lambda) \mathbf{y_{j\textit{sub}}}$\\
            // \textit{\textbf{replace the original sequences}}\\
            \For{k in \left\{ i, j\right\}}
            {
                 $\tilde{\mathbf{x_{k}}} = \mathbf{x}_k - \mathbf{x_{k\textit{sub}}} + \tilde{\mathbf{x_{\textit{sub}}}}$\\
                  $\tilde{\mathbf{y_{k}}} = \mathbf{y}_k - \mathbf{y_{k\textit{sub}}} + \tilde{\mathbf{y_{\textit{sub}}}}$\\
                   \If{$d(\left\langle \tilde{\mathbf{x_k}}, \tilde{\mathbf{y_k}} \right\rangle)$}
                    {
                        $\mathcal{L}^* = \mathcal{L}^* \cup \left\langle \tilde{\mathbf{x_k}}, \tilde{\mathbf{y_k}} \right\rangle$\\
                    }   
                    \If{$|\mathcal{L}^*| \geq N $}{break}
            }
        }
}

 \KwOut{Generated sequences and labels $\mathcal{L}^*$}
 \caption{SeqMix}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%5%





==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
